Multi-Agent Influence Diagrams to Hybrid Threat Modeling

Western governments have adopted an assortment of counter-hybrid threat measures to defend against hostile actions below the conventional military threshold. The impact of these measures is unclear because of the ambiguity of hybrid threats, their cross-domain nature, and uncertainty about how countermeasures shape adversarial behavior. This paper offers a novel approach to clarifying this impact by unifying previously bifurcating hybrid threat modeling methods through a (multi-agent) influence diagram framework. The model balances the costs of countermeasures, their ability to dissuade the adversary from executing hybrid threats, and their potential to mitigate the impact of hybrid threats. We run 1000 semi-synthetic variants of a real-world-inspired scenario simulating the strategic interaction between attacking agent A and defending agent B over a cyber attack on critical infrastructure to explore the effectiveness of a set of five different counter-hybrid threat measures. Counter-hybrid measures range from strengthening resilience and denial of the adversary's ability to execute a hybrid threat to dissuasion through the threat of punishment. Our analysis primarily evaluates the overarching characteristics of counter-hybrid threat measures. This approach allows us to generalize the effectiveness of these measures and examine parameter impact sensitivity. In addition, we discuss policy relevance and outline future research avenues.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}
\mycomment{
\bibitem{Gelman2011}
Gelman, A. (2011). Causality and statistical learning.

\bibitem{Bareinboim2020a}
Bareinboim, E., Correa, J. D., Ibeling, D., and Icard, T. (2020). On Pearl’s hierarchy and the foundations of causal inference. ACM Special Volume in Honor of Judea Pearl (provisional title), 2(3), 4.

\bibitem{Bareinboim2012} Bareinboim, E., Brito, C., and Pearl, J. (2012). Local characterizations of causal Bayesian networks. In Graph Structures for Knowledge Representation and Reasoning (pp. 1-17). Springer, Berlin, Heidelberg.

\bibitem{Glymour2019}
Glymour, C., Zhang, K., and Spirtes, P. (2019). Review of causal discovery methods based on graphical models. Frontiers in genetics, 10, 524.

\bibitem{Pearl2009b}
Pearl, J. (2009). Causal inference in statistics: An overview. Statistics surveys, 3, 96-146.


\bibitem{Chickering2003}
Chickering, D. M. (2003). Optimal structure identification with greedy search. J. Mach. Learn. Res. 3, 507–554. doi: 10.1162/153244303321897717

\bibitem{Guo2020a}
Guo, R., Cheng, L., Li, J., Hahn, P. R., and Liu, H. (2020). A survey of learning causality with data: Problems and methods. ACM Computing Surveys (CSUR), 53(4), 1-37.

\bibitem{Ogburn2014}
Ogburn, E. L., and VanderWeele, T. J. (2014). Causal diagrams for interference. Statistical science, 29(4), 559-578.

\bibitem{Aronow2017} Aronow, P. M., and Samii, C. (2017). Estimating average causal effects under general interference, with application to a social network experiment. The Annals of Applied Statistics, 11(4), 1912-1947.

\bibitem{Pearl2009a} Pearl, J. (2009). Causality. Cambridge university press.

\bibitem{Cole2009} Cole, S. R., and Frangakis, C. E. (2009). The consistency statement in causal inference: a definition or an assumption?. Epidemiology, 20(1), 3-5.

\bibitem{Colombo2012} Colombo, D., Maathuis, M. H., Kalisch, M., and Richardson, T. S. (2012). Learning high-dimensional directed acyclic graphs with latent and selection variables. The Annals of Statistics, 294-321.

\bibitem{Weele2009} VanderWeele, T. J. (2009). Concerning the consistency assumption in causal inference. Epidemiology, 20(6), 880-883.

\bibitem{Peters2017} Peters, J., Janzing, D., and Schölkopf, B. (2017). Elements of causal inference: foundations and learning algorithms (p. 288). The MIT Press.

\bibitem{Richardson2002} Richardson, T., and Spirtes, P. (2002). Ancestral graph Markov models. The Annals of Statistics, 30(4), 962-1030.

\bibitem{Koller2009} Koller, D., Friedman, N. (2009). Probabilistic graphical models: principles and techniques. MIT press.


\bibitem{Salmer2018} Salmer on, A., Rum i, R., Langseth, H., Nielsen, T. D., and Madsen, A.L. (2018). A review of inference algorithms for hybrid Bayesian networks. Journal of Artificial Intelligence Research, 62, 799-828.

\bibitem{Langseth2009} Langseth, H., Nielsen, T. D., Rum, R., and Salmeron, A. (2009). Inference in hybrid Bayesian networks. Reliability Engineering and System Safety,
94(10), 1499-1509

\bibitem{Hanea2015} Hanea, A., Napoles, O. M., and Ababei, D. (2015). Non-parametric Bayesian networks: Improving theory and reviewing applications. Reliability Engineering System Safety, 144, 265-284.

\bibitem{Sherman2018} Sherman, E., and Shpitser, I. (2018). Identification and estimation of causal effects from dependent data. Advances in neural information processing systems, 31.

\bibitem{Shenoy2011} Shenoy, P. P., and West, J. C. (2011). Inference in hybrid Bayesian net-works using mixtures of polynomials. International Journal of Approximate Reasoning, 52(5), 641-657

\bibitem{Ihler2012} Chen, S. H., and Pollino, C. A. (2012). Good practice in Bayesian network modelling. Environmental Modelling and Software, 37, 134-145.

\bibitem{Pearl1995} Pearl, J. (1995). Causal diagrams for empirical research. Biometrika, 82(4), 669-688.

\bibitem{Shpitser2006} Shpitser, I., and Pearl, J. (2006). Identification of joint interventional distributions in recursive semi-Markovian causal models (pp. 1219-1226). eScholarship, University of California.

\bibitem{Bareinboim2020b} Correa, J., and Bareinboim, E. (2020, April). A calculus for stochastic interventions: Causal effect identification and surrogate experiments. In Proceedings of the AAAI conference on artificial intelligence (Vol. 34, No. 06, pp. 10093-10100).

\bibitem{Shpitser2016} Shpitser, I., and Tchetgen, E. T. (2016). Causal inference with a graphical hierarchy of interventions. Annals of statistics, 44(6), 2433.

\bibitem{Malinsky2019} Malinsky, D., Shpitser, I., and Richardson, T. (2019, April). A potential outcomes calculus for identifying conditional path-specific effects. In The 22nd International Conference on Artificial Intelligence and Statistics (pp. 3080-3088). PMLR.

\bibitem{Bhattacharya2020} Bhattacharya, R., Malinsky, D., and Shpitser, I. (2020, August). Causal inference under interference and network uncertainty. In Uncertainty in Artificial Intelligence (pp. 1028-1038). PMLR.

\bibitem{Dawid2000} Dawid, A. P. (2000). Causal inference without counterfactuals. Journal of the American statistical Association, 95(450), 407-424.

\bibitem{Richardson2013a} Richardson, T. S., and Robins, J. M. (2013, July). Single world intervention graphs: a primer. In Second UAI workshop on causal structure learning, Bellevue, Washington.

\bibitem{Richardson2013b} Richardson, T. S., and Robins, J. M. (2013). Single world intervention graphs (SWIGs): A unification of the counterfactual and graphical approaches to causality. Center for the Statistics and the Social Sciences, University of Washington Series. Working Paper, 128(30), 2013.


\bibitem{Young2014} Young, J. G., Hernán, M. A., and Robins, J. M. (2014). Identification, estimation and approximation of risk under interventions that depend on the natural value of treatment using observational data. Epidemiologic methods, 3(1), 1-19.

\bibitem{Soto2020} Soto, M. G., Sucar, L. E., and Escalante, H. J. (2020). Causal Games and Causal Nash Equilibrium. Research in Computing Science, 149, 123-133.

\bibitem{Grimbly2021} Grimbly, S. J., Shock, J., and Pretorius, A. (2021). Causal Multi-Agent Reinforcement Learning: Review and Open Problems. arXiv preprint arXiv:2111.06721.

\bibitem{Maes2007} Maes, S., Meganck, S., and Manderick, B. (2007). Inference in multi-agent causal models. International journal of approximate reasoning, 46(2), 274-299.

\bibitem{Weele2013} VanderWeele, T. J., and Hernan, M. A. (2013). Causal inference under multiple versions of treatment. Journal of causal inference, 1(1), 1-20.

\bibitem{Runge2018} Runge, J. (2018). Causal network reconstruction from time series: From theoretical assumptions to practical estimation. Chaos: An Interdisciplinary Journal of Nonlinear Science, 28(7), 075310.

\bibitem{Zhang2016} Zhang, J., and Spirtes, P. (2016). The three faces of faithfulness. Synthese, 193(4), 1011-1027.

\bibitem{Cox1958} Cox, D. R. (1958). Planning of experiments.

\bibitem{Imbens2010} Imbens, G. W., and Rubin, D. B. (2010). Rubin causal model. In Microeconometrics (pp. 229-241). Palgrave Macmillan, London.

\bibitem{Rubin1974} Rubin, D. B. (1974). Estimating causal effects of treatments in randomized and nonrandomized studies. Journal of educational Psychology, 66(5), 688.

\bibitem{Rubin1978} Rubin, D. B. (1978). Bayesian inference for causal effects: The role of randomization. The Annals of statistics, 34-58.

\bibitem{Rosenbaum1983} Rosenbaum, P. R., and Rubin, D. B. (1983). The central role of the propensity score in observational studies for causal effects. Biometrika, 70(1), 41-55.

\bibitem{Holland1986} Holland, P. W. (1986). Statistics and causal inference. Journal of the American statistical Association, 81(396), 945-960.

\bibitem{Nichols2007} Nichols, A. (2007). Causal inference with observational data. The Stata Journal, 7(4), 507-541.

\bibitem{Byron1972} Byron, R. P. (1972). Testing for misspecification in econometric systems using full information. International Economic Review, 745-756.

\bibitem{Sorbom1975} Sörbom, D. (1975). Detection of correlated errors in longitudinal data. British Journal of Mathematical and Statistical Psychology, 28(2), 138-151.

\bibitem{Wermuth1982} Wermuth, N., and Lauritzen, S. L. (1982). Graphical and recursive models for contigency tables. Institut for Elektroniske Systemer, Aalborg Universitetscenter.

\bibitem{Spirtes1990} Spirtes, P., Glymour, C., and Scheines, R. (1990). causality from probability, proceedings of Advanced Computing for the Social Sciences. Williamsburgh, VA.

\bibitem{Spirtes1991} Spirtes, P., and Glymour, C. (1991). An algorithm for fast recovery of sparse causal graphs. Social science computer review, 9(1), 62-72.

\bibitem{Shimizu2006} Shimizu, S., Hoyer, P. O., Hyvärinen, A., Kerminen, A., and Jordan, M. (2006). A linear non-Gaussian acyclic model for causal discovery. Journal of Machine Learning Research, 7(10).

\bibitem{Shimizu2011} Shimizu, S., Inazumi, T., Sogawa, Y., Hyvärinen, A., Kawahara, Y., Washio, T., ... and Bollen, K. (2011). DirectLiNGAM: A direct method for learning a linear non-Gaussian structural equation model. The Journal of Machine Learning Research, 12, 1225-1248.

\bibitem{Zhang2012} Zhang, K., and Hyvarinen, A. (2012). On the identifiability of the post-nonlinear causal model. arXiv preprint arXiv:1205.2599.

\bibitem{Hoyer2008a} Hoyer, P. O., Shimizu, S., Kerminen, A. J., and Palviainen, M. (2008). Estimation of causal effects using linear non-Gaussian causal models with hidden variables. International Journal of Approximate Reasoning, 49(2), 362-378.

\bibitem{Hoyer2008b} Hoyer, P., Janzing, D., Mooij, J. M., Peters, J., and Schölkopf, B. (2008). Nonlinear causal discovery with additive noise models. Advances in neural information processing systems, 21.

\bibitem{Lacerda2012} Lacerda, G., Spirtes, P. L., Ramsey, J., and Hoyer, P. O. (2012). Discovering cyclic causal models by independent components analysis. arXiv preprint arXiv:1206.3273.

\bibitem{Bongers2021} Bongers, S., Forré, P., Peters, J., and Mooij, J. M. (2021). Foundations of structural causal models with cycles and latent variables. The Annals of Statistics, 49(5), 2885-2915.

\bibitem{Molina2014} Molina, J., Pantazis, L., and Sued, M. (2014). Some considerations on the back door theorem and conditional randomization. Epidemiologic Methods, 3(1), 113-120.

\bibitem{Malinsky2018} Malinsky, D., and Danks, D. (2018). Causal discovery algorithms: A practical guide. Philosophy Compass, 13(1), e12470.

\bibitem{Goudet2019} Goudet, O., Kalainathan, D., Sebag, M., and Guyon, I. (2019). Learning bivariate functional causal models. In Cause effect pairs in machine learning (pp. 101-153). Springer, Cham.

\bibitem{Spirtes2004} Spirtes, P., and Scheines, R. (2004). Causal inference of ambiguous manipulations. Philosophy of Science, 71(5), 833-845.

\bibitem{Spirtes2000} Spirtes, P., Glymour, C. N., Scheines, R., and Heckerman, D. (2000). Causation, prediction, and search. MIT press.

\bibitem{Ogarrio2016} Ogarrio, J. M., Spirtes, P., and Ramsey, J. (2016, August). A hybrid causal search algorithm for latent variable models. In Conference on probabilistic graphical models (pp. 368-379). PMLR.

\bibitem{Eberhardt2009} Eberhardt, F. (2009). Introduction to the Epistemology of Causation. Philosophy Compass, 4(6), 913-925.

\bibitem{Pena2016} Peña, J. M. (2016, August). Learning acyclic directed mixed graphs from observations and interventions. In Conference on Probabilistic Graphical Models (pp. 392-402). PMLR.

\bibitem{Tchetgen2012} Tchetgen, E. J. T., and VanderWeele, T. J. (2012). On causal inference in the presence of interference. Statistical methods in medical research, 21(1), 55-75.

\bibitem{Hudgens2008} Hudgens, M. G., and Halloran, M. E. (2008). Toward causal inference with interference. Journal of the American Statistical Association, 103(482), 832-842.

\bibitem{Lauritzen2002} Lauritzen, S. L., and Richardson, T. S. (2002). Chain graph models and their causal interpretations. Journal of the Royal Statistical Society: Series B (Statistical Methodology), 64(3), 321-348.

\bibitem{Maier2013a} Maier, M., Marazopoulou, K., Arbour, D., and Jensen, D. (2013). A sound and complete algorithm for learning causal models from relational data. arXiv preprint arXiv:1309.6843.

\bibitem{Maier2013b} Maier, M., Marazopoulou, K., and Jensen, D. (2013). Reasoning about independence in probabilistic models of relational data. arXiv preprint arXiv:1302.4381.

\bibitem{Arbour2016} Arbour, D., Garant, D., and Jensen, D. (2016, August). Inferring network effects from observational data. In Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining (pp. 715-724).

\bibitem{Shpitser2015} Shpitser, I. (2015). Segregated graphs and marginals of chain graph models. Advances in neural information processing systems, 28.

\bibitem{Andersson2001} Andersson, S. A., Madigan, D., and Perlman, M. D. (2001). Alternative Markov properties for chain graphs. Scandinavian journal of statistics, 28(1), 33-85.

\bibitem{Lauritzen1996} Lauritzen, S. L. (1996). Graphical models: Oxford University Press.[Google Scholar].

\bibitem{Duarte2021} Duarte, E., and Solus, L. (2021). Representation and Learning of Context-Specific Causal Models with Observational and Interventional Data. arXiv preprint arXiv:2101.09271.

\bibitem{Geiger1996} Geiger, D., and Heckerman, D. (1996). Knowledge representation and inference in similarity networks and Bayesian multinets. Artificial Intelligence, 82(1-2), 45-74.

\bibitem{Boutilier2013} Boutilier, C., Friedman, N., Goldszmidt, M., and Koller, D. (2013). Context-specific independence in Bayesian networks. arXiv preprint arXiv:1302.3562.

\bibitem{Smith2008} Smith, J. Q., and Anderson, P. E. (2008). Conditional independence and chain event graphs. Artificial Intelligence, 172(1), 42-68.

\bibitem{Pensar2015} Pensar, J., Nyman, H., Koski, T., and Corander, J. (2015). Labeled directed acyclic graphs: a generalization of context-specific independence in directed graphical models. Data mining and knowledge discovery, 29(2), 503-533.

\bibitem{Hyttinen2018} Hyttinen, A., Pensar, J., Kontinen, J., and Corander, J. (2018, August). Structure learning for Bayesian networks over labeled DAGs. In International Conference on Probabilistic Graphical Models (pp. 133-144). PMLR.

\bibitem{Leonelli2021} Leonelli, M., and Varando, G. (2021). Context-Specific Causal Discovery for Categorical Data Using Staged Trees. arXiv preprint arXiv:2106.04416.

\bibitem{Carli2020} Carli, F., Leonelli, M., Riccomagno, E., and Varando, G. (2020). The R package stagedtrees for structural learning of stratified staged trees. arXiv preprint arXiv:2004.06459.

\bibitem{Beuzen2018} Beuzen, T., Marshall, L., and Splinter, K. D. (2018). A comparison of methods for discretizing continuous variables in Bayesian Networks. Environmental Modelling and Software: with Environment Data News, 108, 61–66.

\bibitem{Granger1969} Granger, C. W. (1969). Investigating causal relations by econometric models and cross-spectral methods. Econometrica: journal of the Econometric Society, 424-438.

\bibitem{Verma1990} Verma, T. S., and Pearl, J. (1990). Equivalence and synthesis of causal models. In Probabilistic and Causal Inference: The Works of Judea Pearl (pp. 221-236).


\bibitem{Zhang2011} Zhang, J., and Spirtes, P. (2011). Intervention, determinism, and the causal minimality condition. Synthese, 182(3), 335-347.

\bibitem{Peters2014} Peters, J., Mooij, J. M., Janzing, D., and Schölkopf, B. (2014). Causal discovery with continuous additive noise models.

\bibitem{Gibbard1978} Gibbard, A., and Harper, W. L. (1978). Counterfactuals and two kinds of expected utility. In Ifs (pp. 153-190). Springer, Dordrecht.

\bibitem{Robins1986} Robins, J. (1986). A new approach to causal inference in mortality studies with a sustained exposure period—application to control of the healthy worker survivor effect. Mathematical Modelling, 7(9), 1393–1512.

\bibitem{Shpitser2022} Shpitser, I., Richardson, T. S., and Robins, J. M. (2022). Multivariate counterfactual systems and causal graphical models. In Probabilistic and Causal Inference: The Works of Judea Pearl (pp. 813-852).

\bibitem{Robins2010} Robins, J. M., and Richardson, T. S. (2010). Alternative graphical causal models and the identification of direct effects. Causality and psychopathology: Finding the determinants of disorders and their cures, 84, 103-158.

\bibitem{Robins2022} Robins, J. M., Richardson, T. S., and Shpitser, I. (2022). An interventionist approach to mediation analysis. In Probabilistic and Causal Inference: The Works of Judea Pearl (pp. 713-764).

\bibitem{Cox2000} Cox, P. M., Betts, R. A., Jones, C. D., Spall, S. A., and Totterdell, I. J. (2000). Acceleration of global warming due to carbon-cycle feedbacks in a coupled climate model. Nature, 408(6809), 184-187.

\bibitem{Richardson2017} Richardson, T. S., Evans, R. J., Robins, J. M., and Shpitser, I. (2017). Nested Markov properties for acyclic directed mixed graphs. arXiv preprint arXiv:1701.06686.

\bibitem{Tikka2019} Tikka, S., Hyttinen, A., and Karvanen, J. (2019). Identifying causal effects via context-specific independence relations. Advances in neural information processing systems, 32.

\bibitem{Richardson2014} Richardson, T. S. (2014). A factorization criterion for acyclic directed mixed graphs. arXiv preprint arXiv:1406.6764.

%\bibitem{Robins2004} Robins, J. M., Hernán, M. A., and SiEBERT, U. W. E. (2004). Effects of multiple interventions. Comparative quantification of health risks: global and regional burden of disease attributable to selected major risk factors, 1, 2191-2230.

\bibitem{Yao2021} Yao, L., Chu, Z., Li, S., Li, Y., Gao, J., and Zhang, A. (2021). A survey on causal inference. ACM Transactions on Knowledge Discovery from Data (TKDD), 15(5), 1-46.

\bibitem{Stuart2010} Stuart, E. A. (2010). Matching methods for causal inference: A review and a look forward. Statistical science: a review journal of the Institute of Mathematical Statistics, 25(1), 1.

\bibitem{DAmour2021} D’Amour, A., Ding, P., Feller, A., Lei, L., and Sekhon, J. (2021). Overlap in observational studies with high-dimensional covariates. Journal of Econometrics, 221(2), 644-654.

\bibitem{Assaad2022} Assaad, C. K., Devijver, E., and Gaussier, E. (2022). Survey and Evaluation of Causal Discovery Methods for Time Series. Journal of Artificial Intelligence Research, 73, 767-819.

\bibitem{Vowels2021} Vowels, M. J., Camgoz, N. C., and Bowden, R. (2021). D'ya like dags? a survey on structure learning and causal discovery. arXiv preprint arXiv:2103.02582.

\bibitem{Yu2016} Yu, K., Li, J., and Liu, L. (2016). A review on algorithms for constraint-based causal discovery. arXiv preprint arXiv:1611.03977.

\bibitem{Yuan2007} Yuan, C., and Druzdzel, M. J. (2007, March). Importance sampling for general hybrid Bayesian networks. In Artificial intelligence and statistics (pp. 652-659). PMLR.

\bibitem{Nogueira2021} Nogueira, A. R., Gama, J., and Ferreira, C. A. (2021). Causal discovery in machine learning: Theories and applications. Journal of Dynamics and Games, 8(3), 203.

\bibitem{Andersen2013} Andersen, H. (2013). When to expect violations of causal faithfulness and why it matters. Philosophy of Science, 80(5), 672-683.

\bibitem{Hausman1999} Hausman, D. M., and Woodward, J. (1999). Independence, invariance and the causal Markov condition. The British journal for the philosophy of science, 50(4), 521-583.

\bibitem{Cartwright1999} Cartwright, N. (1999). Causal diversity and the Markov condition. Synthese, 3-27.

\bibitem{Ramsey2017} Ramsey, J., Glymour, M., Sanchez-Romero, R., and Glymour, C. (2017). A million variables and more: the fast greedy equivalence search algorithm for learning high-dimensional graphical causal models, with an application to functional magnetic resonance images. International journal of data science and analytics, 3(2), 121-129.

\bibitem{Zhang2013} Zhang, J. (2013). A comparison of three occam's razors for markovian causal models. The British journal for the philosophy of science, 64(2), 423-448.

\bibitem{Forster2020} Forster, M., Raskutti, G., Stern, R., and Weinberger, N. (2020). The frugal inference of causal relations. The British Journal for the Philosophy of Science.

\bibitem{Marx2021} Marx, A., Gretton, A., and Mooij, J. M. (2021, December). A weaker faithfulness assumption based on triple interactions. In Uncertainty in Artificial Intelligence (pp. 451-460). PMLR.

\bibitem{Humphreys1996} Humphreys, P., and Freedman, D. (1996). The grand leap. The British journal for the philosophy of science, 47(1), 113-123.

\bibitem{Korb1997} Korb, K. B., and Wallace, C. S. (1997). In search of the philosopher's stone: remarks on Humphreys and Freedman's critique of causal discovery. The British journal for the philosophy of science, 48(4), 543-553.

\bibitem{Freedman1999} Freedman, D., and Humphreys, P. (1999). Are there algorithms that discover causal structure?. Synthese, 121(1), 29-54.

\bibitem{Dawid2010} Dawid, A. P. (2010, February). Beware of the DAG!. In Causality: objectives and assessment (pp. 59-86). PMLR.

\bibitem{Guo2020b} Guo, R., Li, J., and Liu, H. (2020, January). Learning individual causal effects from networked observational data. In Proceedings of the 13th International Conference on Web Search and Data Mining (pp. 232-240).

\bibitem{Hartford2017} Hartford, J., Lewis, G., Leyton-Brown, K., and Taddy, M. (2017, July). Deep IV: A flexible approach for counterfactual prediction. In International Conference on Machine Learning (pp. 1414-1423). PMLR.

\bibitem{Louizos2017} Louizos, C., Shalit, U., Mooij, J. M., Sontag, D., Zemel, R., and Welling, M. (2017). Causal effect inference with deep latent-variable models. Advances in neural information processing systems, 30.

\bibitem{Imbens2015} Imbens, G. W., and Rubin, D. B. (2015). Causal inference in statistics, social, and biomedical sciences. Cambridge University Press.

\bibitem{Nogueira2022} Nogueira, A. R., Pugnana, A., Ruggieri, S., Pedreschi, D., and Gama, J. (2022). Methods and tools for causal discovery and causal inference. Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery, e1449.

\bibitem{Eberhardt2017} Eberhardt, F. (2017). Introduction to the foundations of causal discovery. International Journal of Data Science and Analytics, 3(2), 81-91.

\bibitem{Eberhardt2007} Eberhardt, F., and Scheines, R. (2007). Interventions and causal inference. Philosophy of science, 74(5), 981-995.

\bibitem{Grosz2020} Grosz, M. P., Rohrer, J. M., and Thoemmes, F. (2020). The taboo against explicit causal inference in nonexperimental psychology. Perspectives on Psychological Science, 15(5), 1243-1255.

\bibitem{Rubin1980} Rubin, D. B. (1980). Randomization analysis of experimental data: The Fisher randomization test comment. Journal of the American statistical association, 75(371), 591-593.

\bibitem{Hauser2015} Hauser, A., and Bühlmann, P. (2015). Jointly interventional and observational data: estimation of interventional Markov equivalence classes of directed acyclic graphs. Journal of the Royal Statistical Society: Series B (Statistical Methodology), 77(1), 291-318.

\bibitem{Silva2016} Silva, R. (2016). Observational-interventional priors for dose-response learning. Advances in Neural Information Processing Systems, 29.

\bibitem{Mahmood2011} Mahmood, A. (2011). Structure learning of causal bayesian networks: A survey.

\bibitem{Shalit2020} Shalit, U. (2020). Can we learn individual-level treatment policies from clinical data?. Biostatistics, 21(2), 359-362.

\bibitem{Kreif2019} Kreif, N., and DiazOrdaz, K. (2019). Machine learning in policy evaluation: new tools for causal inference. arXiv preprint arXiv:1903.00402.

\bibitem{Sobel2014} Sobel, D. M., and Legare, C. H. (2014). Causal learning in children. Wiley Interdisciplinary Reviews: Cognitive Science, 5(4), 413-427.

\bibitem{Halloran1995} Halloran, M. E., and Struchiner, C. J. (1995). Causal inference in infectious diseases. Epidemiology, 142-151.
}
\end{thebibliography}


